A New Linear Programming Approach and a New Backtracking Strategy for Multiple-Gradient Descent in Multi-Objective Optimization

In this work, the author presents a novel method for finding descent directions shared by two or more differentiable functions defined on the same unconstrained domain space. Then, the author illustrates an alternative Multiple-Gradient Descent procedure for Multi-Objective Optimization problems that is based on this new method. In particular, the proposed method consists in finding the shared descent direction solving a relatively cheap Linear Programming (LP) problem, where the LP's objective function and the constraints are defined by the gradients of the objective functions of the Multi-Objective Optimization problem. More precisely, the formulation of the LP problem is such that, if a shared descent direction does not exist for the objective functions, but a non-ascent direction for all the objectives does, the LP problem returns the latter. Moreover, the author defines a new backtracking strategy for Multiple-Gradient Descent methods such that, if the proposed LP is used for computing the direction, the ability to reach and/or explore the Pareto set and the Pareto front is improved. A theoretical analysis of the properties of the new methods is performed, and tests on classic Multi-Objective Optimization problems are proposed to assess their goodness.

==> NewCommands/Francesco.commands.tex <==
% (CREDO) COMANDI "SCONSIGLIATI" MA DA USARE IN CASO DI CAPITOLI NON NUMERATI DA INSERIRE NEL'INDICE
%
%\newcommand{\addchap}[1]{\addcontentsline{toc}{chapter}{{#1}}}
%\newcommand{\addsec}[1]{\addcontentsline{toc}{section}{{#1}}}

\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\fra}[1]{{\color{violet}#1}}
\newcommand{\mgnt}[1]{{\color{magenta}#1}}

==> NewCommands/Francesco.defaultoptions.tex <==
%%% BIBLATEX %%%
\usepackage[backend=biber,style=numeric-comp,citestyle=numeric,sorting=nty,natbib,maxbibnames=10]{biblatex}
%%%%%%%%%%%%%%%%%%%%%%%

%%% GRAFICHE %%%
\usepackage{graphicx}
% TIKZ %
\usepackage{tikz}
% PGFPLOTS %
\usepackage{pgfplots}
\pgfplotsset{compat=1.6}%{width=10cm, compat=1.9} % retrocompatibilità e proprietà varie plot
\usepgfplotslibrary{groupplots}
% VELOCIZZAZIONE/RETROCOMPATIBILITA' PGFPLOTS (CREA PDF CHE POI CARICA) - NON SEMPRE FUNZIONA %
% \usepgfplotslibrary{external}
% \tikzexternalize
% GRAFI CON TIKZ (richiede tikz)%
\usepackage{pgf}
\usetikzlibrary{positioning,shapes,arrows,fit,calc,automata}
% PACKAGE FOR DRAWING NNs (UP-TO-DATE PACKAGE NOT ON CTAN BUT ON https://github.com/battlesnake/neural) %
\usepackage{neuralnetwork}
% PACKAGE FOR NETWORK DRAWINGS (ALSO 3D!!)
\usepackage{tikz-network}

%%% LINGUA %%%
\usepackage[english]{babel}

%%% A4WIDE OPTION %%%%%%%
\usepackage{a4wide}

%%% SPAZIO INTORNO A SEZIONE & SIMILI %%%
%\usepackage{titlesec}
%%FUNZIONAMENTO GENERALE:
%%\titlespacing*{<command>}{<left>}{<before-sep>}{<after-sep>}
%% ESEMPI (USATO IN TESI PhD):
%\titlespacing*{\section}
%{0pt}{3\baselineskip}{1.5\baselineskip}

%%% SUPPORTO UNICODE %%%
%\usepackage{ucs}      % SEMBRA NON SERVIRE
% \usepackage[utf8x]{inputenc}
% IN TOPTESI NON FUNZIONANO... (A COSA SERVIVANO?)
% \SetUnicodeOption{mathletters}
% \SetUnicodeOption{autogenerated}
%%%%%%%%%%%%%%%%%%%%%%%

%%% SIMBOLI %%%
\usepackage{amsmath, amsthm, amsfonts, amssymb}
\usepackage{mathabx}   % upup-..-dowdow arrows
\usepackage[makeroom]{cancel}    % cancellation symbol
\usepackage{tipa}      % fonetica
\usepackage{textcomp}  % caratteri extra
\usepackage{latexsym}  % simboli vari
\usepackage{mathrsfs}  % caratteri corsivi (agg. io); per utilizzarlo: \mathscr{•}
%%%%%%%%%%%%%


%%% LUNGHEZZA DELL'INDENTAZIONE (se 0 non c'è)%%%
\setlength{\parindent}{3mm}


%% NOMENCLATURA %%%
%\usepackage[intoc]{nomencl}
%\makenomenclature
% Importazione opzioni per gruppi di nomenclature
% \input{ReferencesAndNomenclatures/GroupsNomenclature.tex}
% PER STAMPARE LA NOMENCLATURA:
%- fare un file .tex con all'interno varie voci del tipo: \nomenclature[group]{symbol}{description}
%- importare il file .tex (dove si vuole)
%- scrivere il comando \printnomenclature dove si vuole che venga stampata la nomenclatura
% ATTENZIONE: in toptesi la nomenclatura viene "letta" solo se inserita nel main matter!
%%%%%%%%%%%%%%%%%%%


%%% ENUMITEM CON NUMERAZIONE "STILE SEZIONI" %%%
% per numerazioni 1.1,1.2,... nell'ambiente ENUMERATE quando ne metto uno dentro all'altro
\renewcommand{\labelenumii}{\theenumii}
\renewcommand{\theenumii}{\theenumi.\arabic{enumii}.}

%credo oppure (metterlo nella cartella come per 'mcode'):
\usepackage{enumitem}% http://ctan.org/pkg/enumitem
% e utilizzare così:
%\begin{enumerate}
%  \item First
%  \begin{enumerate}[label*=\arabic*.]
%    \item Second
%    \item Third
%  \end{enumerate}
%  \item Fourth
%\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% PACCHETTO PER LINK A REF  %%%
\usepackage{hyperref}
\hypersetup{
	%bookmarks=true,         % show bookmarks bar?
	%unicode=false,          % non-Latin characters in Acrobat’s bookmarks
	%pdftoolbar=true,        % show Acrobat’s toolbar?
	%pdfmenubar=true,        % show Acrobat’s menu?
	%pdffitwindow=false,     % window fit to page when opened
	%pdfstartview={FitH},    % fits the width of the page to the window
	%pdftitle={My title},    % title
	%pdfauthor={Author},     % author
	%pdfsubject={Subject},   % subject of the document
	%pdfcreator={Creator},   % creator of the document
	%pdfproducer={Producer}, % producer of the document
	%pdfkeywords={keyword1, key2, key3}, % list of keywords
	%pdfnewwindow=true,      % links in new PDF window
	colorlinks=true,       % false: boxed links; true: colored links
	linkcolor=blue,%red,          % color of internal links (change box color with linkbordercolor)
	citecolor=red,%green,        % color of links to bibliography
	filecolor=magenta,      % color of file links
	urlcolor=cyan           % color of external links
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% CLEVEREF PACKAGE FOR \Cref, \cref, ecc. %%%
\usepackage{cleveref}

%%% PERSONALIZZAZIONE STILE TABELLE %%%
% PACCHETTO PER HLINE IN TABELLE
\usepackage{hhline}
% FATT. MOLTIPLICATIVO ALTEZZA TABELLE (Valore standard 1.2)
\renewcommand\arraystretch{1.5}
% ALTRI PACCHETTI PER TABELLE (MULTIRIGHE E COLORI)
\usepackage{multirow}
\usepackage{colortbl} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%% PACCHETTI PER ALGORITMI IN PSEUDOCODICE %%%
\usepackage{algpseudocode}
\usepackage{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% PACCHETTO PER CORREZIONI %%%
\usepackage{cancel}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% ---- COLORAZIONE DIMOSTRAZIONI (commentare per non colorarle) ---
%\usepackage{etoolbox}
%\usepackage{xcolor}
%\usepackage{amsthm}
%\AtBeginEnvironment{proof}{\color{lightgray}}
%%% -----------------------------------------


%%% --- PACCHETTO PER SOTTOFIGURE CON CAPTION DEDICATA ---
\usepackage{subcaption} 
% utilizzo: 
% \begin{figure}[htb]
%     \centering
%     \subcaptionbox{caption figura 1}{\includegraphics[width=0.44\textwidth]{Figura1.png}}
% 	\subcaptionbox{caption figura 2}{\includegraphics[width=0.44\textwidth]{Figura2.png}}
%     \caption{caption generale}
%     \label{fig:figura}
% \end{figure}





==> NewCommands/Francesco.newtheorems.tex <==
%Stile CORSIVO per i 'newtheorem' successivi

%ambiente 'teo' con la scritta 'Theorem' e numerazione subordinata alla sezione
\newtheorem{teo}{Theorem}[section]

%ambiente 'prop' con la scritta 'Proposition' e numerazione subordinata alla sezione
\newtheorem{prop}{Proposition}[section]

%ambiente 'cor' con la scritta 'Corollary' e numerazione uguale al teorema
\newtheorem{cor}[teo]{Corollary}

%ambiente 'lem' con la scritta 'Lemma' e numerazione subordinata alla sezione
\newtheorem{lem}{Lemma}[section]

%ambiente 'defin' con la scritta 'Definition' e numerazione subordinata alla sezione
\newtheorem{defin}{Definition}[section]

%ambiente 'sch' con la scritta 'Scheme' e numerazione subordinata alla sezione
\newtheorem{sch}{Scheme}[section]

%ambiente 'prin' con la scritta 'Principle' e numerazione subordinata alla sezione
\newtheorem{prin}{Principle}[section]

%ambiente 'ex' con la scritta 'Exercise' e numerazione subordinata alla sezione
\newtheorem{ex}{Exercise}[section]

%ambiente 'notaz' con la scritta 'Notation' e numerazione subordinata alla sezione
\newtheorem{notaz}{Notation}[section]

%ambiente 'alg' con la scritta 'Algoritmo' e numerazione subordinata alla sezione
\newtheorem{alg}{Algorithm}[section]



%Stile diverso (NON CORSIVO) per i 'newtheorem' successivi
\theoremstyle{definition}

%ambiente 'oss' con la scritta 'Observation' e numerazione subordinata alla sezione
\newtheorem{oss}{Observation}[section]

%ambiente 'oss' con la scritta 'Observation' e numerazione subordinata alla sezione
\newtheorem{rem}{Remark}[section]

%ambiente 'prog' con la scritta 'Program' e numerazione subordinata alla sezione
\newtheorem{prog}{Program}[section]

%ambiente 'es' con la scritta 'Example' e numerazione subordinata alla sezione
\newtheorem{es}{Example}[section]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> NewCommands/Francesco.symbols.tex <==
%%% PACCHETTO PER SWITCH CASES IN newcommand %%%
\usepackage{xstring}
% Example:
% \newcommand{\tree}[2]{%
%     \IfEqCase{#1}{%
%         {a}{$\sqrt{#2}$}%
%         {b}{Hi}%
%         % you can add more cases here as desired
%     }[\PackageError{tree}{Undefined option to tree: #1}{}]%
% }%

%%% PACCHETTO PER IF/ELSE CASES IN newcommand
\usepackage{ifthen}
% In brief: \ifthenelse{test}{then clause}{else clause}



%%% FACCIAMO POSTO PER LE SCORCIATOIE SUCCESSIVE %%%

\newcommand{\dOld}{\d}
\newcommand{\sOld}{\s}
\newcommand{\lOld}{\l}
\newcommand{\rOld}{\r}
\newcommand{\vOld}{\v}
\newcommand{\tOld}{\t}
\newcommand{\bOld}{\b}
\newcommand{\cOld}{\c}
\newcommand{\kOld}{\k}
% \newcommand{\COld}{\C}

%%% SEMPLIFICAZIONE DELLA SINTASSI E SCORCIATOIE %%%

\newcommand{\TENS}[1]{\mathop{\mathbf{#1}}\nolimits} % Tensori (lettere maiuscole)
\newcommand{\Dkl}[2]{D_{\mathrm{KL}}\left({#1}\parallel{#2}\right)}	% Divergenza di Kullback-Liebler
\newcommand{\Djs}[2]{D_{\mathrm{JS}}\left({#1}, {#2}\right)}	% Divergenza di Jensen-Shannon
\newcommand{\herm}[1]{{#1}^\dagger}	% Hermitiana di matrice
\newcommand{\trasp}[1]{{#1}^\top}	% Trasposta di matrice
\newcommand{\norm}[1]{\parallel{#1}\parallel}	% Norma
\newcommand{\eps}{\varepsilon}				%   eps: la vecchia varepsilon
\renewcommand{\d}{\mathrm{d}}					%   d:	differenziale
\newcommand{\f}{\frac}							%   f:	frazione
\newcommand{\tf}{\tfrac}						%  tf:	frazione piccola
\renewcommand{\s}{\sqrt}						%   s:	radice
\newcommand{\pd}[2]{\f{∂{#1}}{∂{#2}}}					%  pd:	derivata parziale
\newcommand{\pdd}[2]{\f{∂^2{#1}}{∂{#2}^2}}				% pdd:	derivata parziale seconda
\newcommand{\td}[2]{\f{\d{#1}}{\d{#2}}}					%  td:	derivata totale
\newcommand{\tdd}[2]{\f{\d^2{#1}}{\d{#2}^2}}				% tdd:	derivata totale seconda
\newcommand{\fd}[2]{\f{δ{#1}}{δ{#2}}}					%  fd:	derivata funzionale
\newcommand{\pq}{\overleftrightarrow{∂}}				%  pq:  derivata parziale $bidirezionale$
\renewcommand{\l}{\left}						%   l:	left
\renewcommand{\r}{\right}						%   r:	right
\renewcommand{\v}{\ensuremath{\boldsymbol}}				%   v:	vettore (grassetto) [MEGLIO \boldsymbol O \pmb ?]
\renewcommand{\t}{\text}						%   t:	text
\newcommand{\I}{\indices}						%   I:	indici tensoriali (pacchetto tensor)
\newcommand{\h}{\ensuremath{\hbar}}					%   h:	h tagliato
\newcommand{\ccall}{\ensuremath{\mathcal}}				%   c:  calligrafico
% \renewcommand{\C}{\ensuremath{\mathbb{C}}}				%   C:  insieme dei numeri complessi
\newcommand{\C}{\ensuremath{\mathbb{C}}}				%   C:  insieme dei numeri complessi

\newcommand{\N}{\ensuremath{\mathbb{N}}}				%   N:  insieme dei numeri naturali
\newcommand{\R}{\ensuremath{\mathbb{R}}}				%   R:  insieme dei numeri Reali
\newcommand{\Q}{\ensuremath{\mathbb{Q}}}				%   Q:  insieme dei numeri Razionali
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}				%   Z:  insieme dei numeri Interi
\renewcommand{\k}[1]{\ensuremath{\mathinner{|{#1}\rangle}}}		%   k:	|⋅>
\renewcommand{\b}[1]{\ensuremath{\mathinner{\langle{#1}|}}}		%   b:	<⋅|
\newcommand{\bk}[1]{\ensuremath{\mathinner{\langle{#1}\rangle}}}	%  bk:  <⋅>
\newcommand{\bkt}[2]{\mathinner{\langle{#1}|{#2}\rangle}}		% bkt:  <⋅|⋅>
\newcommand{\B}[1]{\left\langle#1\right|}				%   B:  |⋅>     scaling
\newcommand{\K}[1]{\left|#1\right\rangle}				%   K:  <⋅|     scaling
\newcommand{\BK}[1]{\left\langle{#1}\right\rangle}			%  BK:  <⋅>     scaling
\newcommand{\BKT}[2]{\left\langle{#1}\mid{#2}\right\rangle}		% BKT:  <⋅|⋅>   scaling
\newcommand{\wt}{\widetilde}						%  td:	widetilde
\newcommand{\ol}{\overline}
\newcommand{\bsy}{\boldsymbol}		                % abbreviation for math boldsymbol 

%%% OPERATORI MATEMATICI %%% (aggiungere ad ogni necessità)
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Corr}{Corr}
\DeclareMathOperator{\argmin}{arg\,min}
\DeclareMathOperator{\argmax}{arg\,max}
\DeclareMathOperator{\E}{\ensuremath{\mathbb{E}}}				%   E:  Valore Atteso
\DeclareMathOperator{\sigm}{sigm}
\DeclareMathOperator{\relu}{relu}
\DeclareMathOperator{\elu}{elu}
\DeclareMathOperator{\softp}{softp}
\DeclareMathOperator{\swish}{swish}
\DeclareMathOperator{\softm}{softmax}
\DeclareMathOperator{\depth}{depth}

%%%%%%%%%%%%% T O D O %%%%%%%%%%%%%%%
% includere \bb{} al posto di \mathbb{}. Contestualmente scegliere uno da http://www.latex-community.org/forum/viewtopic.php?f=5&t=2238 (link in fondo). Deve funzionare anche \bb{1}

%%% Se si vuole nabla vettore... %%%
%\let\nablino\nabla
%\renewcommand{\nabla}{\boldsymbol{\nablino}}


==> NewCommands/dfn.symbols.tex <==
\newcommand{\CAL}[1]{\mathop{\cal {#1}}\nolimits}
% GIA' IN Francesco.symbols.tex
%\newcommand{\TENS}[1]{\mathop{\mathbf{#1}}\nolimits}
\newcommand{\Si}{\CAL{S}_i}
\newcommand{\jumpS}[1]{\mathop{\left[\negthickspace\left[#1\right]\negthickspace\right]_{S}}\nolimits}
\newcommand{\jumpSm}[1]{\mathop{ \left[\negthickspace\left[#1\right]\negthickspace\right]_{S_m} }\nolimits}
\newcommand{\sobh}[2]{\mathop{{\rm H}^{#1}{\rm (}#2{\rm )}}\nolimits}
